Bayesian Inverse Graphics for Few-Shot Concept Learning

Humans excel at building generalizations of new concepts from just one single example. Contrary to this, current computer vision models typically require large amount of training samples to achieve a comparable accuracy. In this work we present a Bayesian model of perception that learns using only minimal data, a prototypical probabilistic program of an object. Specifically, we propose a generative inverse graphics model of primitive shapes, to infer posterior distributions over physically consistent parameters from one or several images. We show how this representation can be used for downstream tasks such as few-shot classification and pose estimation. Our model outperforms existing few-shot neural-only classification algorithms and demonstrates generalization across varying lighting conditions, backgrounds, and out-of-distribution shapes. By design, our model is uncertainty-aware and uses our new differentiable renderer for optimizing global scene parameters through gradient descent, sampling posterior distributions over object parameters with Markov Chain Monte Carlo (MCMC), and using a neural based likelihood function.

==> sections/priors.tex <==
We now proceed to explain our PGM and it's probabilistic variables $\ProbabilisticParameters = \{ \Shift, \Angle, \Scale, \Color, \Ambient, \Diffuse, \Specular, \Shininess, \Classes \}$.
The prior selected for the object translation $\Shift$ is a truncated Gaussian distribution ($\mathrm{Tr}\mathcal{N}$) with its limits determined such that the translation of an object has the highest probability mass in the middle of the image plane and 0 mass outside of it.
The prior of the angle $\Angle$ across the object's the z-axis was selected using a von Mises distribution which assigns equal probability to all angles.
The object scales are sampled from a Log-normal ($\mathrm{Log}\mathcal{N}$) distribution that doesn't consider negative scales, or extremely small or large objects.
The prior distribution $\Classes$ for the shape classes $\{\mathrm{sphere}, \mathrm{cube}, \mathrm{cylinder} \}$ is a Gumbel-Softmax distribution ($\mathrm{Gmb}$)~\cite{jang2016categorical}, which locates most of the probability mass as one-hot vectors instead of uniformly distributed classes.
The rationale being that objects should not be simultaneously multiple classes at once.
The parameters and distributions of all our priors are shown in the supplementary Section~\ref{sec:supp_priors}.
%\noindent \textbf{Data-driven priors:}
Furthermore, through our scene optimization procedure in Section~\ref{sec:scene_optimization} we obtained point estimates for the material properties 
$\Scene_{\Object} = \{
    \Color_{j},
    \Ambient_{j},
    \Diffuse_{j},
    \Specular_{j},
    \Shininess_{j}
\}$
across all $j$ training objects.
We used these optimized parameters to build single prior distributions for each of those same variables $\Color$, $\Ambient$, $\Diffuse$, $\Specular$, $\Shininess$.
These training data driven priors were fitted using a Gaussian Mixture Model (GMM) using expectation maximization (EM).
For each variable we use 2 mixture components with a diagonal covariance matrix.
All GMM prior models are shown in the supplementary Section~\ref{sec:data_driven_priors_results}.


==> sections/probabilistic_generative_model.tex <==
%\noindent \textbf{Probabilistic generative model:}
Having defined our prior distributions, we proceed to build a probabilistic generative model of images.
Figure~\ref{fig:probabilistic_program} shows our model in plate notation and Figure~\ref{fig:prior_predictive_samples} shows its prior predictive samples.
These prior predictive samples reflect what the model expects to see before making any observation.
Moreover, our model outputs a probability for each sample.
This all being referred as the prior predictive distribution (PPD).
We now proceed to explain in detail the probability density functions (PDFs) and the deterministic functions applied to our model.

\begin{figure}[t!]
    \begin{subfigure}[b]{0.60\linewidth}
        \centering
        \input{sections/images/probabilistic_program}
        \caption{Probabilistic inverse graphics model}~\label{fig:probabilistic_program}
    \end{subfigure}
    \begin{subfigure}[b]{0.40\linewidth}
        \centering
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/25_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/00_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/32_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/10_prior_predictive_sample.png}
        \end{subfigure}

        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/51_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/82_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/61_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/simple/56_prior_predictive_sample.png}
        \end{subfigure}

        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/dark/58_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/dark/27_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/dark/23_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/dark/99_prior_predictive_sample.png}
        \end{subfigure}

        \begin{subfigure}[b]{0.235\textwidth}
            \includegraphics[width=\textwidth]{images/prior_predictive_samples/room/36_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\textwidth]{images/prior_predictive_samples/room/42_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\textwidth]{images/prior_predictive_samples/room/76_prior_predictive_sample.png}
        \end{subfigure}
        \begin{subfigure}[b]{0.235\linewidth}
            \includegraphics[width=\linewidth]{images/prior_predictive_samples/room/74_prior_predictive_sample.png}
        \end{subfigure}
        \caption{Prior predictive samples}~\label{fig:prior_predictive_samples}
    \end{subfigure} 
    \caption{Inverse graphics model and prior predictive samples for \fsclvr, \fsclvrdark, and the \fsclvrroom~datasets}~\label{fig:inverse_graphics_model}
    \vspace{-0.30cm}
\end{figure}

We define the (PDF) over possible materials $\Material$ by considering each property material $M = \{\Color, \Ambient, \Diffuse, \Specular, \Shininess \}$ as independent:
\begin{equation}\label{eq:pdf_material}
    p(\Material|\Color, \Ambient, \Diffuse, \Specular, \Shininess) =
        \prod_{m \in M} \left[ \sum_{k=0}^{K} \pi_{k}^{m} \mathcal{N}(m | \mu_k^{m}, \Sigma_{k}^{m}) \right]
\end{equation}
As shown in Figure~\ref{fig:probabilistic_program} the PDF over possible affine transformations $\GenerativeTransform$ includes a $\TruncatedNormalDistribution$, von Mises, and a $\LogNormalDistribution$~distribution, and considers the translation, angle and scale as independent events:
%\begin{equation}~\label{eq:pdf_transform}
    %\begin{align}
   %p(\GenerativeTransform | \Shift, \Angle, \Scale) = 
%   \prod_{t}^{T} \mathrm{Tr}\mathcal{N}(\Shift | \mu_t, \sigma_t)
   %\prod_{t}^{T} \left[ \frac{\mathcal{N}(\Shift | \mu_t, \sigma_t)}{\Phi \left(\frac{b - \mu_{t}}{\sigma_{t}} \right) - \Phi \left(\frac{a - \mu_{t}}{\sigma_{t}} \right)} \right] \\ 
%    \frac{\exp(\kappa \cos(\theta - \mu_{\theta})) }{2\pi I_0(\kappa)} \prod_{s}^{S}
%    \frac{ \exp(-\frac{(\ln(s) - \mu_{s})^2}{2 \sigma_{s}^{2}} ) }{s \sigma_{s} \sqrt{2 \pi}} 
    %\end{align}
%\end{equation}
\begin{equation}~\label{eq:pdf_transform}
   p(\GenerativeTransform | \Shift, \Angle, \Scale) = 
   \prod_{t \in T} \left[ \frac{\TruncatedNormalDistribution(\Shift | \mu_t, \sigma_t)}{2\pi I_0(0)} \right]
   \prod_{s \in S} \frac{ \exp(-\frac{(\ln(s) - \mu_{s})^2}{2 \sigma_{s}^{2}} ) }{s \sigma_{s} \sqrt{2 \pi}}
    %\end{align}
\end{equation}
where $T = \{x, y \}$, $S = \{ s_x, s_y, s_z \}$ and $I_0$ is the Bessel function of order zero.
Finally, we compute the probability density function over objects $p(\GenerativeObject | \Material, \GenerativeShape, \GenerativeTransform) $ using the previously defined PDFs for materials~\ref{eq:pdf_material} and transforms~\ref{eq:pdf_transform}, as well as $p(\Classes  | \bm{\sigma}, \mathrm{t})$ corresponding to the Gumbel-Softmax probability with a class probability $\bm{\sigma}$ and a temperature $t$.
\begin{equation}
    p(\Classes | \bm{\sigma}, \mathrm{t})
    p(\Material | \Color, \Ambient, \Diffuse, \Specular, \Shininess)
    p(\GenerativeTransform | \Shift, \Angle, \Scale)
\end{equation}
Furthermore, the object variable $\GenerativeObject$ is passed through our deterministic differentiable rendering function $\DiffGraphics$ outputting image samples, and similarly to~\cite{gothoskar20213dp3} we build an affine transform that enforces objects to not collide with the floor.
%Similarly as in~\cite{gothoskar20213dp3}, we enforce that objects do not collide with the reconstructed scene, by building the affine transform $T$ such that the object is translated in the $z$ direction equally to the sampled z-scale $s_z$.
%This affine transformation is given explicitly as:
%\begin{equation}
%    \GenerativeTransform=
%    \begin{bmatrix}
%        1 & 0 & 0 & x \\
%        0 & 1 & 0 & y \\
%        0 & 0 & 1 & s_z \\
%        0 & 0 & 0 & 1 \\
%    \end{bmatrix}
%    \begin{bmatrix}
%        \cos(\Angle) & -\sin{\Angle} & 0 & 0 \\
%        \sin(\Angle) & \cos{\Angle} & 0 & 0 \\
%        0 & 0 & 1 & 0 \\
%        0 & 0 & 0 & 1 \\
%    \end{bmatrix}
%    \begin{bmatrix}
%        s_x & 0 & 0 & 0 \\
%        0 & s_y & 0 & 0 \\
%        0 & 0 & s_z & 0 \\
%        0 & 0 & 0 & 1 \\
%    \end{bmatrix}
%\end{equation}
%Having defined a forward generative model of images, we now proceed to perform Bayesian inference in order to obtain the posterior distribution of our parameters $\ProbabilisticParameters = \{ \Shift, \Angle, \Scale, \Color, \Ambient, \Diffuse, \Specular, \Shininess, \Classes \}$ given an observation $\Observation$.
Having defined a forward generative model of images, we now perform Bayesian inference in order to obtain the posterior distributions over the variables $\ProbabilisticParameters$ given an observation $\Observation$.

\begin{equation}
    p(\ProbabilisticParameters | \Observation) \sim p(\Observation | \ProbabilisticParameters) p(\ProbabilisticParameters)\label{eqn:target_probability}
\end{equation}
%Where $\ProbabilisticParameters = \{ \Shift, \Angle, \Scale, \Color, \Ambient, \Diffuse, \Specular, \Shininess, \GenerativeProbabilities \}$.
%We define a likelihood using a truncated normal distribution over each pixel:
We define a color likelihood function $\ColorLikelihood$ using a truncated normal distribution over each pixel argument $(u, v, c)$ of an image $\Observation$ with shape [H, W, 3]:
%\begin{equation}
%    \Likelihood(u, v | \Omega) = \prod_{u}^{W} \prod_{v}^{H} = \frac{\phi\left(\frac{x - \mu}{\sigma}\right)}{\Phi\left(\frac{b - \mu}{\sigma}\right) - \Phi\left(\frac{a - \mu}{\sigma}\right)}
%\end{equation}
\begin{equation}
\xi(u, v, c) = \Render(u, v, c | \ProbabilisticParameters) - \ImageData(u, v, c)
\end{equation}
\begin{equation}~\label{eq:color_likelihood}
    \Likelihood(u, v | \ProbabilisticParameters)_{\mathrm{C}} =
        \prod_{u=0}^{W} \prod_{v=0}^{H} \prod_{c=0}^{3} \mathrm{Tr}\mathcal{N}(\xi(u, v, c), \sigma_{I}) \\
\end{equation}
%\begin{equation}
%    \Phi(x) = \frac{1}{2}(1 + \mathrm{erf}(x / \sqrt(2)))
%\end{equation}
All parameters of our PGM are displayed in the supplementary Section~\ref{sec:supp_priors}.
%Both our neural~\ref{eq:neural_likelihood} and color likelihood~\ref{eq:color_likelihood} functions only consider RGB images, with no depth information.
% We consider this property useful for ubiquitous robotic applications.
Given our target probability function, and an observation $\Observation$, we can now sample from a conditioned posterior distribution using MCMC. \\


==> sections/probabilistic_prototypical_programs.tex <==
In this section we reuse the posterior samples to build a prototypical object representation.
Specifically, we perform a Gaussian kernel density estimate (KDE) using Scott's bandwidth~\cite{scott1992density} for the posterior samples of the variables $\Scale$, $\Ambient$, $\Diffuse$, $\Specular$, $\Shininess$ and $\Classes$.
Thus, our prototypical representation consists of all our previous posterior samples excluding the pose variables $\Shift$ and $\theta$.
%These posterior distributions form a generative model of objects
These posterior distributions are used to build a new generative model by removing these variables from our previous inverse graphics model~\ref{fig:probabilistic_program}.
A visualization of this new graphical model is shown in the supplementary Section~\ref{sec:supplementary_prototypical}.
Moreover, we define the functions \distance~and \merge~between two generative models.
We define the \textit{distance} between two generative models $C_I$ and $C_k$ as the sum of the Kullback-Leibler divergences across our selected variables $\ProtoVariables = \{ \Scale, \Ambient, \Diffuse, \Specular, \Shininess, \Classes \}$:
\begin{equation}
    d(C_{I}, C_{k}) =
        \sum_{\ProtoVariables} \text{KL}(C_{k}^{\ProtoVariables} \| C_{I}^{\ProtoVariables}) =
        \sum_{\psi} \sum_{x} C_{k}^{\psi}(x) \log \frac{C_{k}^{\ProtoVariables}(x)}{C_{I}^{\ProtoVariables}(x)}
\end{equation}
The \merge~operation ($\otimes$) is defined as performing KDE on the concatenated posterior samples for each variable in both PGMs.
We define this conditioned probabilistic generative models with these two additional functions as a protoprogram $C$.
Moreover, protoprograms have the additional functionalities associated to all PGMs; those being the capacity to \texttt{sample}~and to compute the \texttt{probability} of any given sample.
Consequently, protoprograms allow us to generate new concepts and images that are similar to our given prototypical observation.
Figure~\ref{fig:posterior_samples} shows ordered samples of the protoprogram conditioned on observation~\ref{fig:true_test_image}.
This characteristic was indicated to be a relevant human trait that is not present in most few-shot learning methods~\cite{lake2019omniglot}.
Having defined our protoprograms we proceed to present a classification algorithm.
Given $\mathrm{N}$ example images (shots) of an object class $k$, we proceed to build a protoprogram for this class by merging all conditioned programs as $C_k = C_1^{k} \otimes C_{2}^{k} \otimes \ldots C_{\mathrm{N}}^{k}$.
Given a new observation $I$, we proceed to learn a program $C_{I}$ following the same structure as before.
We then use the program \textit{distance} to compute a probability conditioned on each protoprogram class by applying softmax on the negative program distances.

\begin{equation}
	p(c=k | I) = \frac{\exp(-d(C_{I}, C_{k}))}{\sum_{k} \exp(-d(C_{I}, C_{k}))}\label{eqn:softmax}
\end{equation}


==> sections/results/dark.tex <==
\begin{tabular}{lcccc}
        \hline
        \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
        & \textbf{1-shot}    & \textbf{5-shot} & \textbf{1-shot}    & \textbf{5-shot}  \\
        %\textbf{Model}   & \textbf{5-way 1-shot}    & \textbf{5-way 5-shot} & \textbf{10-way 1-shot}    & \textbf{10-way 5-shot}  \\
        \hline
        $\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 79.56\% & 86.22\%  & 60.39\%  & 62.77\%  \\
        $\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 69.08\% & 80.36\%  & 49.15\%  & 63.00\%  \\
        $\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 65.34\% & 86.66\%  & 52.88\%  & 79.32\%  \\
        $\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 43.92\% & 70.58\%  & 32.51\%  & 58.19\%  \\  
 		\hline
        P3 (ours) & 96.86\%  & 98.04\%  & 93.88\%  & 96.62\%  \\
        NP3 (ours) & \textbf{97.30\%}  & \textbf{98.48\%}  & \textbf{94.88\%}  & \textbf{97.31\%}  \\
 		\hline
\end{tabular}


==> sections/results/global_results.tex <==
\begin{tabular}{l|cccc|cccc}
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\underline{\textbf{\fsclvr~test dataset}}} & \multicolumn{4}{c}{\underline{\textbf{\fsclvrroom~test dataset}}} \\
& \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c|}{\textbf{10-way}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
& \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
\hline
$\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 76.96\% & 87.48\% & 62.82\% & 69.84\% & 77.94\% & 79.18\% & 47.23\% & 61.46\% \\
$\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 70.86\% & 32.38\% & 51.77\% & 64.95\% & 72.96\% & 81.72\% & 32.12\% & 57.01\% \\
$\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 60.52\% & 85.54\% & 51.22\% & 79.73\% & 66.70\% & 83.04\% & 54.65\% & 72.18\% \\
$\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 51.16\% & 74.94\% & 40.13\% & 67.09\% & 47.12\% & 68.32\% & 33.65\% & 54.41\% \\
\hline
P3 (ours) & 95.98\% & \textbf{98.98\%} & 92.61\% & \textbf{97.51\%} & 91.66\% & 96.98\% & 86.01\% & 93.59\% \\
NP3 (ours) & \textbf{97.18\%} & 98.86\% & \textbf{94.52\%} & 97.47\% & \textbf{94.36\%} & \textbf{98.96\%} & \textbf{90.52\%} & \textbf{97.53\%} \\
\hline
\hline
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\underline{\textbf{\fsclvr~test dataset}}} & \multicolumn{4}{c}{\underline{\textbf{\fsclvrroom~test dataset}}} \\
& \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c|}{\textbf{10-way}} & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
& \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} & \textbf{1-shot} & \textbf{5-shot} \\
\hline
$\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 76.96\% & 87.48\% & 62.82\% & 69.84\% & 77.94\% & 79.18\% & 47.23\% & 61.46\% \\
$\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 70.86\% & 32.38\% & 51.77\% & 64.95\% & 72.96\% & 81.72\% & 32.12\% & 57.01\% \\
$\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 60.52\% & 85.54\% & 51.22\% & 79.73\% & 66.70\% & 83.04\% & 54.65\% & 72.18\% \\
$\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 51.16\% & 74.94\% & 40.13\% & 67.09\% & 47.12\% & 68.32\% & 33.65\% & 54.41\% \\
\hline
P3 (ours) & 95.98\% & \textbf{98.98\%} & 92.61\% & \textbf{97.51\%} & 91.66\% & 96.98\% & 86.01\% & 93.59\% \\
NP3 (ours) & \textbf{97.18\%} & 98.86\% & \textbf{94.52\%} & 97.47\% & \textbf{94.36\%} & \textbf{98.96\%} & \textbf{90.52\%} & \textbf{97.53\%} \\
\hline
\end{tabular}


==> sections/results/plain.tex <==
\begin{tabular}{lcccc}
        \hline
        \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
        & \textbf{1-shot}    & \textbf{5-shot} & \textbf{1-shot}    & \textbf{5-shot}  \\
        %\textbf{Model}   & \textbf{5-way 1-shot}    & \textbf{5-way 5-shot} & \textbf{10-way 1-shot}    & \textbf{10-way 5-shot}  \\
        \hline
        $\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 76.96\% & 87.48\%  & 62.82\%  & 69.84\%  \\
        $\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 70.86\% & 32.38\%  & 51.77\%  & 64.95\%  \\
        $\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 60.52\% & 85.54\%  & 51.22\%  & 79.73\%  \\
        $\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 51.16\% & 74.94\%  & 40.13\%  & 67.09\%  \\
        \hline
        P3 (ours) & 95.98\%  & \textbf{98.98\%}  & 92.61\%  & \textbf{97.51\%}  \\
        NP3 (ours) & \textbf{97.18\%}  & 98.86\%  & \textbf{94.52\%}  & 97.47\%  \\
 		\hline
\end{tabular}


==> sections/results/room.tex <==
\begin{tabular}{lcccc}
        \hline
        \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
        & \textbf{1-shot}    & \textbf{5-shot} & \textbf{1-shot}    & \textbf{5-shot}  \\
        %\textbf{Model}   & \textbf{5-way 1-shot}    & \textbf{5-way 5-shot} & \textbf{10-way 1-shot}    & \textbf{10-way 5-shot}  \\
        \hline
        $\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 77.94\% & 79.18\%  & 47.23\%  & 61.46\%  \\
        $\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 72.96\% & 81.72\%  & 32.12\%  & 57.01\%  \\
        $\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 66.70\% & 83.04\%  & 54.65\%  & 72.18\%  \\
        $\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 47.12\% & 68.32\%  & 33.65\%  & 54.41\%  \\  
        \hline
        P3 (ours) & 91.66\%  & 96.98\%  & 86.01\%  & 93.59\%  \\
        NP3 (ours) & \textbf{94.36\%}  & \textbf{98.96\%}  & \textbf{90.52\%}  & \textbf{97.53\%}  \\
 		%TRIDENT & 23.31\%  & 40.26\%  & 10.00\%  & 9.27\%  \\
 		\hline
\end{tabular}


==> sections/results/ycbood.tex <==
\begin{tabular}{lcccc}
        \hline
        \multirow{2}{*}{\textbf{Model}}   & \multicolumn{2}{c}{\textbf{5-way}} & \multicolumn{2}{c}{\textbf{10-way}} \\
        & \textbf{1-shot}    & \textbf{5-shot} & \textbf{1-shot}    & \textbf{5-shot}  \\
        %\textbf{Model}   & \textbf{5-way 1-shot}    & \textbf{5-way 5-shot} & \textbf{10-way 1-shot}    & \textbf{10-way 5-shot}  \\ \hline
        $\textrm{MAML}_{56 \times 56}$~\cite{finn2017model} & 47.22\% & 32.70\%  & 36.55\%  & 39.16\%  \\
        $\textrm{MAML}_{84 \times 84}$~\cite{finn2017model} & 52.22\% & 37.56\%  & 39.83\%  & 47.56\%  \\
        %\hline
        $\textrm{ProtoNets}_{56 \times 56}$~\cite{snell2017prototypical} & 49.80\% & 67.26\%  & 39.13\%  & 57.37\%  \\
        $\textrm{ProtoNets}_{84 \times 84}$~\cite{snell2017prototypical} & 41.26\% & 62.28\%  & 30.96\%  & 50.33\%  \\
 		\hline
        P3 (ours) & 66.42\%  & 67.84\%  & 60.32\%  & 57.31\%  \\
        NP3 (ours) & \textbf{67.44}\%  & \textbf{71.26}\%  & \textbf{62.09}\%  & \textbf{61.36}\%  \\
 		\hline
\end{tabular}


==> sections/scene_optimization_data_driven.tex <==
While maximizing realism does close the simulation-reality gap, there are still elements for which our differentiable renderer is unable to match perfectly with the true images.
These elements are related to soft shadows, material reflections and different shape topologies.
Thus, we propose a neural metric that measures image discrepancy in feature space.
We apply this neural metric as a likelihood function when fitting a probabilistic graphical model using MCMC.
Using a neural network within MCMC implies performing a forward pass for every sample; moreover, not all featuremaps are relevant for all tasks.
%Thus, we opted to use only those feature maps $\Featuremap$ that remain invariant between our rendered images $\Render$ and the true images $\ImageData$.
Thus, we opted to use only those channels $\FeatureChannel$ of the feature maps $\Featuremap$ that remain invariant between our rendered images $\Render$ and the true images $\ImageData$
\begin{equation}
    \Featuremap_{\FeatureChannel}(\Render) \approx \Featuremap_{\FeatureChannel}(\ImageData).
\end{equation}
This implies that we use only those neural features that map similar images to similar feature values.
To construct this invariant transformation we compute the mean square error across all feature maps channels $\FeatureChannel$ of VGG16~\cite{simonyan2014very}.
%To construct this invariant transformation we solved the following optimization problem for all layers $l$ and feature maps channels $m$ of VGG16~\cite{simonyan2014very}.
%\begin{equation}
    %\argmin_{m, l} {\| \Featuremap_{m}^{l}(I_R, \theta) - \Featuremap_{m}^{l}(I, \theta) \|}_{2}
%    \argmin_{m, l} \frac{{\| \Featuremap_{m}^{l}(I_R, \theta) - \Featuremap_{m}^{l}(I, \theta) \|}_{2}}{N(m, l)}
%\end{equation}
% Where $N(m, l)$ correponds to the number of 
We choose this network due to both its fast inference time, and its widespread application as a feature extraction model~\cite{zhang2018unreasonable}.
Moreover, our methodology is generic and can be applied to any deep learning model.
%Moreover, without loss of generality, our methodology can be applied to any deep learning model.
% Specifically, we use our previously optimized scenes $s \in S$ to compute the accumulated loss for each feature map channel across all convolutional layers:
Specifically, we used the training pairs of true images and the previously optimized image scenes $(\ImageData, \Render^{*}) \in \ImagePairSet$ to compute the accumulated loss for each feature map channel $\FeatureChannel$:
\begin{equation}
    \mathcal{L}(\FeatureChannel) = \frac{1}{\FeaturemapSize(\FeatureChannel)} \sum_{(\ImageData, \Render^{*}) \in \ImagePairSet} {\| \Featuremap_{\FeatureChannel}(\Render^{*}) - \Featuremap_{\FeatureChannel}(\ImageData) \|}_{2}
\end{equation}
where $\FeaturemapSize(\FeatureChannel)$ indicates the number of pixel features in channel $\FeatureChannel$.
We select the feature channels $\FeatureChannel^{*} \in \OptimalFeatureChannelSet$ that accumulate the least amount of loss across the training image pairs $\ImagePairSet$.
% The results containing the top-K channels across the first 8 convolutional layers can be seen in Table~\ref{tab:neural_likelihood}.
For the \fsclvr~training the top 3 channels correspond to the 25th, 51th and 2nd of the 1st convolution layer.
This result is computationally favorable since we can extract the first layer of our model and use it during sampling.
%Furthermore, we consider every feature pixel $u$, $v$ and feature channels $m^{*}$ as independent; thus, the general formulation of our neural likelihood function is of the form:
%Furthermore, we consider as independent the pixel pairs $(u, v)$ of the feature image $I_{m^{*}}$ of every channel $m^{*}$.
%Thus, the general formulation of our neural likelihood function is of the form:
%Furthermore, we consider as independent the pixel pairs $(u, v)$ of the feature image $I_{m^{*}}$ of every channel $m^{*}$.
%Thus, the general formulation of our neural likelihood function is of the form:
With the optimized feature channels $\FeatureChannel^{*}$ with pixel feature arguments $n$ we build the neural likelihood function $\NeuralLikelihood$ with respect to some hypothesis $\ProbabilisticParameters$ and an observation $\Observation$ as:
\begin{equation}~\label{eq:neural_likelihood}
    \NeuralLikelihood(\Observation | \ProbabilisticParameters) \propto
    \prod_{\FeatureChannel^{*} \in \OptimalFeatureChannelSet} \prod_{n=0}^{\FeaturemapSize(\FeatureChannel^{*})}
    \exp(
        \Featuremap_{\FeatureChannel^{*}}^{n}(\Observation)) -
        \Featuremap_{\FeatureChannel^{*}}^{n}(\Render(\ProbabilisticParameters))
\end{equation}
%\begin{equation}~\label{eq:neural_likelihood}
%    \Likelihood_{m, u, v} \propto
%    \prod_{m^{*} \in M} \prod_{(u, v) \in I_{m^{*}}}
%    \exp(\Featuremap_{m^{*}}(I_{R})(u,v) - \Featuremap_{m^{*}}(I)(u, v))
%\end{equation}
% Interestingly, feature maps located at the end of the CNN tend to have more error.
%Figure~\ref{fig:neural_likelihood} shows our final neural likelihood.
%We observe how similar those feature map channels look, independently of the material conditions, and light and floor differences within the true scene.


==> sections/scene_optimization_model_based.tex <==
In order to minimize the simulation-reality gap we maximize realism between our generative model and the training dataset.
We do this by optimizing the scene parameters
$\Scene = \{
    \Shift_{k},
    \LightIntensity_{k},
    \Color_{\Floor},
    \Pattern_{\Floor},
    \Ambient_{\Floor},
    \Diffuse_{\Floor},
    \Color_{j},
    \Ambient_{j},
    \Diffuse_{j},
    \Specular_{j},
    \Shininess_{j}
\}$ with gradient descent through our differentiable renderer.
%as shown in Figure~\ref{fig:differentiable_scene_optimization}.
These parameters correspond respectively to the $k$ light positions and light intensities, the floor color, floor pattern, floor ambient, and floor diffuse variables, as well as all $j$ training objects' colors, ambient, diffuse, specular, and shininess properties.
Specifically $\Shift_k, \LightIntensity_k$, $\Color_{\Floor}$ and $\Color_{j}$ $\in \mathbb{R}^3$, $\Pattern_{\Floor}$ $\in  \mathbb{R}^{\text{H} \times \text{W} \times 3}$ and all remaining variables are scalar values.

The reflected color from a realistic material changes with respect to the lighting conditions.
Moreover, the reflected color informs the light parameters about their possible location and intensity.
Thus, we optimized the scene parameters by alternating \texttt{N} gradient updates between global scene parameters
$\Scene_{\Global} = \{ 
    \Shift_{k},
    \LightIntensity_{k},
    \Color_{\Floor},
    \Pattern_{\Floor},
    \Ambient_{\Floor},
    \Diffuse_{\Floor}
\}$
and the object parameters
$\Scene_{\Object} = \{
    \Color_{j},
    \Ambient_{j},
    \Diffuse_{j},
    \Specular_{j},
    \Shininess_{j}
\}$.
We used ADAM with a learning rate of $0.01$ using a $\mathrm{L}_{2}$ loss between our rendered image and the true image.
We alternate gradient updates between $\Scene_{\Global}$ and $\Scene_{\Object}$ with N=7 episodes, $k=5$ and a pattern image of shape $200 \times 200 \times 3$.
% (5 * (3 + 3)) + 3 + (200 * 200 * 3) + (1 + 1) + (30 * (3 + 1 + 1 + 1 + 1)).
In total we optimized 120K parameters, all of which are physically interpretable.
Results of the optimization procedure can be observed in Figure~\ref{fig:model_based_optimization}.
%Each column in these figures corresponds respectively to initial starting condition, episode 1,  episode 7 and the true image.
All material point estimates optimized on the \fsclvr~training set are displayed in Figure~\ref{fig:optimized_materials}.
\begin{figure}[t!]
    \begin{subfigure}[T]{0.5\linewidth}
        \begin{subfigure}{\linewidth}
            \caption{\fsclvr}
            \input{sections/images/scene_optimization_fsclvr}
        \end{subfigure}
        \\ 
        \begin{subfigure}{\linewidth}
            \caption{\fsclvr~optimized train-set materials}~\label{fig:optimized_materials}
            \includegraphics[width=\linewidth]{images/primitives_optimized_materials.png}
        \end{subfigure}
    \end{subfigure}
    \begin{subfigure}[T]{0.5\linewidth}
        \begin{subfigure}{\linewidth}
            \caption{\fsclvrdark}
            \input{sections/images/scene_optimization_fsclvr_dark}
        \end{subfigure}
        \\
        \begin{subfigure}{\linewidth}
            \input{sections/images/scene_optimization_fsclvr_room}
            \caption{\fsclvrroom}
        \end{subfigure}
    \end{subfigure}
    \caption{Model based scene optimization}~\label{fig:model_based_optimization}
    \vspace{-1.0cm}
\end{figure}


==> sections/supplementary_differentiable_rendering.tex <==
\begin{figure}[htpb]
    \begin{subfigure}[T]{0.50\linewidth}
        \includegraphics[width=\linewidth]{images/differentiable_rendering_parameters.pdf}
        \caption{Example of differentiable scene parameters with their respective dimension sizes}~\label{fig:differentiable_rendering_parameters}
    \end{subfigure}
    \begin{subfigure}[T]{0.50\linewidth}
        \input{sections/images/differentiable_rendering_pipeline}
        \caption{Differentiable rendering pipeline}~\label{fig:differentiable_scene_optimization}
    \end{subfigure}
    \caption{Model based scene optimization}~\label{fig:model_based_optimization2}
\end{figure}

